Nonlinear consensus+innovations under correlated heavy-tailed noises: Mean square convergence rate and asymptotics

We consider distributed recursive estimation of consensus+innovations type in the presence of heavy-tailed sensing and communication noises. We allow that the sensing and communication noises are mutually correlated while independent identically distributed (i.i.d.) in time, and that they may both have infinite moments of order higher than one (hence having infinite variances). Such heavy-tailed, infinite-variance noises are highly relevant in practice and are shown to occur, e.g., in dense internet of things (IoT) deployments. We develop a consensus+innovations distributed estimator that employs a general nonlinearity in both consensus and innovations steps to combat the noise. We establish the estimator's almost sure convergence, asymptotic normality, and mean squared error (MSE) convergence. Moreover, we establish and explicitly quantify for the estimator a sublinear MSE convergence rate. We then quantify through analytical examples the effects of the nonlinearity choices and the noises correlation on the system performance. Finally, numerical examples corroborate our findings and verify that the proposed method works in the simultaneous heavy-tail communication-sensing noise setting, while existing methods fail under the same noise conditions.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{caption}
\usepackage{subcaption}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{myassump}{Assumtion}

% Sets running headers as well as PDF title and authors
\headers{Distributed recursive estimation under heavy-tail communication noise}{D. Bajovic, D. Jakovetic, S. Kar, A. K. Sahu and M. Vukovic}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Distributed recursive estimation under heavy-tail communication noise}

% Authors: full names plus addresses.
\author{Dragana Bajovic \thanks{University of Novi Sad, Faculty of Technical Sciences, Department of Power, Electronic and
Communication Engineering
		(\email{dbajovic@uns.ac.rs}).}
\and Dusan Jakovetic\thanks{University of Novi Sad, Faculty of Sciences, Department of Mathematics and Informatics
  (\email{dusan.jakovetic@dmi.uns.ac.rs}).}
\and Soummya Kar\thanks{Department of Electrical and Computer Engineering, Carnegie Mellon University 
	(\email{soummyak@andrew.cmu.edu}).}
\and Anit Kumar Sahu\thanks{Amazon Alexa  AI
	(\email{anit.sahu@gmail.com}).}
\and Manojlo Vukovic\thanks{University of Novi Sad, Faculty of Technical Sciences, Department of Fundamentals Sciences
	(\email{manojlo.vukovic@uns.ac.rs}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Diag}{Diag}
\def\Tr{\mathop{\rm \boldmath Tr}}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

